Systematic Evaluation of LLM-as-a-Judge in LLM Alignment Tasks: Explainable Metrics and Diverse Prompt Templates

LLM-as-a-Judge has been widely applied to evaluate and compare different LLM alignmnet approaches (e.g., RLHF and DPO). However, concerns regarding its reliability have emerged, due to LLM judges' biases and inconsistent decision-making. Previous research has developed evaluation frameworks to assess reliability of LLM judges and their alignment with human preferences. However, the employed evaluation metrics often lack adequate explainability and fail to address LLM internal inconsistency. Additionally, existing studies inadequately explore the impact of various prompt templates when applying LLM-as-a-Judge methods, leading to potentially inconsistent comparisons between different alignment algorithms. In this work, we systematically evaluate LLM-as-a-Judge on alignment tasks by defining more theoretically interpretable evaluation metrics and explicitly mitigating LLM internal inconsistency from reliability metrics. We develop an open-source framework to evaluate, compare, and visualize the reliability and alignment of LLM judges, which facilitates practitioners to choose LLM judges for alignment tasks. In the experiments, we examine effects of diverse prompt templates on LLM-judge reliability and also demonstrate our developed framework by comparing various LLM judges on two common alignment datasets (i.e., TL;DR Summarization and HH-RLHF-Helpfulness). Our results indicate a significant impact of prompt templates on LLM judge performance, as well as a mediocre alignment level between the tested LLM judges and human evaluators.

==> iclr2025_conference.tex <==
@incollection{Bengio+chapter2007,
author = {Bengio, Yoshua and LeCun, Yann},
booktitle = {Large Scale Kernel Machines},
publisher = {MIT Press},
title = {Scaling Learning Algorithms Towards {AI}},
year = {2007}
}

@article{Hinton06,
author = {Hinton, Geoffrey E. and Osindero, Simon and Teh, Yee Whye},
journal = {Neural Computation},
pages = {1527--1554},
title = {A Fast Learning Algorithm for Deep Belief Nets},
volume = {18},
year = {2006}
}

@book{goodfellow2016deep,
title={Deep learning},
author={Goodfellow, Ian and Bengio, Yoshua and Courville, Aaron and Bengio, Yoshua},
volume={1},
year={2016},
publisher={MIT Press}
}

# LLM alignment methods
## HHH criteria
@article{askell2021general,
  title={A general language assistant as a laboratory for alignment},
  author={Askell, Amanda and Bai, Yuntao and Chen, Anna and Drain, Dawn and Ganguli, Deep and Henighan, Tom and Jones, Andy and Joseph, Nicholas and Mann, Ben and DasSarma, Nova and others},
  journal={arXiv preprint arXiv:2112.00861},
  year={2021}
}

## PPO
@article{schulman2017proximal,
  title={Proximal policy optimization algorithms},
  author={Schulman, John and Wolski, Filip and Dhariwal, Prafulla and Radford, Alec and Klimov, Oleg},
  journal={arXiv preprint arXiv:1707.06347},
  year={2017}
}

@article{ouyang2022training,
  title={Training language models to follow instructions with human feedback},
  author={Ouyang, Long and Wu, Jeffrey and Jiang, Xu and Almeida, Diogo and Wainwright, Carroll and Mishkin, Pamela and Zhang, Chong and Agarwal, Sandhini and Slama, Katarina and Ray, Alex and others},
  journal={Advances in neural information processing systems},
  volume={35},
  pages={27730--27744},
  year={2022}
}

@article{bai2022training,
  title={Training a helpful and harmless assistant with reinforcement learning from human feedback},
  author={Bai, Yuntao and Jones, Andy and Ndousse, Kamal and Askell, Amanda and Chen, Anna and DasSarma, Nova and Drain, Dawn and Fort, Stanislav and Ganguli, Deep and Henighan, Tom and others},
  journal={arXiv preprint arXiv:2204.05862},
  year={2022}
}

@article{touvron2023llama,
  title={Llama 2: Open foundation and fine-tuned chat models},
  author={Touvron, Hugo and Martin, Louis and Stone, Kevin and Albert, Peter and Almahairi, Amjad and Babaei, Yasmine and Bashlykov, Nikolay and Batra, Soumya and Bhargava, Prajjwal and Bhosale, Shruti and others},
  journal={arXiv preprint arXiv:2307.09288},
  year={2023}
}

# DPO
@article{rafailov2024direct,
  title={Direct preference optimization: Your language model is secretly a reward model},
  author={Rafailov, Rafael and Sharma, Archit and Mitchell, Eric and Manning, Christopher D and Ermon, Stefano and Finn, Chelsea},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}

@article{yuan2024self,
  title={Self-rewarding language models},
  author={Yuan, Weizhe and Pang, Richard Yuanzhe and Cho, Kyunghyun and Sukhbaatar, Sainbayar and Xu, Jing and Weston, Jason},
  journal={arXiv preprint arXiv:2401.10020},
  year={2024}
}

## best of N (reject sampling)
@article{amini2024variational,
  title={Variational Best-of-N Alignment},
  author={Amini, Afra and Vieira, Tim and Cotterell, Ryan},
  journal={arXiv preprint arXiv:2407.06057},
  year={2024}
}

@article{sessa2024bond,
  title={BOND: Aligning LLMs with Best-of-N Distillation},
  author={Sessa, Pier Giuseppe and Dadashi, Robert and Hussenot, L{\'e}onard and Ferret, Johan and Vieillard, Nino and Ram{\'e}, Alexandre and Shariari, Bobak and Perrin, Sarah and Friesen, Abe and Cideron, Geoffrey and others},
  journal={arXiv preprint arXiv:2407.14622},
  year={2024}
}


# LLM judges that use GPT-4 for win-rate estimation (victims)

# summarizations
@article{wang2024secrets,
  title={Secrets of rlhf in large language models part ii: Reward modeling},
  author={Wang, Binghai and Zheng, Rui and Chen, Lu and Liu, Yan and Dou, Shihan and Huang, Caishuang and Shen, Wei and Jin, Senjie and Zhou, Enyu and Shi, Chenyu and others},
  journal={arXiv preprint arXiv:2401.06080},
  year={2024}
}

@article{huang2024n+,
  title={The N+ Implementation Details of RLHF with PPO: A Case Study on TL; DR Summarization},
  author={Huang, Shengyi and Noukhovitch, Michael and Hosseini, Arian and Rasul, Kashif and Wang, Weixun and Tunstall, Lewis},
  journal={arXiv preprint arXiv:2403.17031},
  year={2024}
}

@article{zhong2024dpo,
  title={Dpo meets ppo: Reinforced token optimization for rlhf},
  author={Zhong, Han and Feng, Guhao and Xiong, Wei and Zhao, Li and He, Di and Bian, Jiang and Wang, Liwei},
  journal={arXiv preprint arXiv:2404.18922},
  year={2024}
}

@article{zheng2023secrets,
  title={Secrets of rlhf in large language models part i: Ppo},
  author={Zheng, Rui and Dou, Shihan and Gao, Songyang and Hua, Yuan and Shen, Wei and Wang, Binghai and Liu, Yan and Jin, Senjie and Liu, Qin and Zhou, Yuhao and others},
  journal={arXiv preprint arXiv:2307.04964},
  year={2023}
}

@article{santacroce2023efficient,
  title={Efficient rlhf: Reducing the memory usage of ppo},
  author={Santacroce, Michael and Lu, Yadong and Yu, Han and Li, Yuanzhi and Shen, Yelong},
  journal={arXiv preprint arXiv:2309.00754},
  year={2023}
}

@article{rafailov2024r,
  title={From $ r $ to $ Q $: Your Language Model is Secretly a Q-Function},
  author={Rafailov, Rafael and Hejna, Joey and Park, Ryan and Finn, Chelsea},
  journal={arXiv preprint arXiv:2404.12358},
  year={2024}
}

# conversations
@article{peng2023stabilizing,
  title={Stabilizing RLHF through advantage model and selective rehearsal},
  author={Peng, Baolin and Song, Linfeng and Tian, Ye and Jin, Lifeng and Mi, Haitao and Yu, Dong},
  journal={arXiv preprint arXiv:2309.10202},
  year={2023}
}

@article{zhu2024proxy,
  title={Proxy-RLHF: Decoupling Generation and Alignment in Large Language Model with Proxy},
  author={Zhu, Yu and Sun, Chuxiong and Yang, Wenfei and Wei, Wenqiang and Tang, Bo and Zhang, Tianzhu and Li, Zhiyu and Zhang, Shifeng and Xiong, Feiyu and Hu, Jie and others},
  journal={arXiv preprint arXiv:2403.04283},
  year={2024}
}

## others
@article{wu2024fine,
  title={Fine-grained human feedback gives better rewards for language model training},
  author={Wu, Zeqiu and Hu, Yushi and Shi, Weijia and Dziri, Nouha and Suhr, Alane and Ammanabrolu, Prithviraj and Smith, Noah A and Ostendorf, Mari and Hajishirzi, Hannaneh},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}

# LLM papers
@article{achiam2023gpt,
  title={Gpt-4 technical report},
  author={Achiam, Josh and Adler, Steven and Agarwal, Sandhini and Ahmad, Lama and Akkaya, Ilge and Aleman, Florencia Leoni and Almeida, Diogo and Altenschmidt, Janko and Altman, Sam and Anadkat, Shyamal and others},
  journal={arXiv preprint arXiv:2303.08774},
  year={2023}
}

@article{anil2023palm,
  title={Palm 2 technical report},
  author={Anil, Rohan and Dai, Andrew M and Firat, Orhan and Johnson, Melvin and Lepikhin, Dmitry and Passos, Alexandre and Shakeri, Siamak and Taropa, Emanuel and Bailey, Paige and Chen, Zhifeng and others},
  journal={arXiv preprint arXiv:2305.10403},
  year={2023}
}

@article{brown2020language,
  title={Language models are few-shot learners},
  author={Brown, Tom B},
  journal={arXiv preprint ArXiv:2005.14165},
  year={2020}
}

## open-source LLMs
@article{dubey2024llama,
  title={The llama 3 herd of models},
  author={Dubey, Abhimanyu and Jauhri, Abhinav and Pandey, Abhinav and Kadian, Abhishek and Al-Dahle, Ahmad and Letman, Aiesha and Mathur, Akhil and Schelten, Alan and Yang, Amy and Fan, Angela and others},
  journal={arXiv preprint arXiv:2407.21783},
  year={2024}
}

# Human evaluation
@article{elangovan2024considers,
  title={ConSiDERS-The-Human Evaluation Framework: Rethinking Human Evaluation for Generative Large Language Models},
  author={Elangovan, Aparna and Liu, Ling and Xu, Lei and Bodapati, Sravan and Roth, Dan},
  journal={arXiv preprint arXiv:2405.18638},
  year={2024}
}

## BACKGROUND 
@article{stureborg2024large,
  title={Large language models are inconsistent and biased evaluators},
  author={Stureborg, Rickard and Alikaniotis, Dimitris and Suhara, Yoshi},
  journal={arXiv preprint arXiv:2405.01724},
  year={2024}
}


# Evaluation of LLM-as-judges

# metrics
@article{wang2023large,
  title={Large language models are not fair evaluators},
  author={Wang, Peiyi and Li, Lei and Chen, Liang and Cai, Zefan and Zhu, Dawei and Lin, Binghuai and Cao, Yunbo and Liu, Qi and Liu, Tianyu and Sui, Zhifang},
  journal={arXiv preprint arXiv:2305.17926},
  year={2023}
}

@article{saito2023verbosity,
  title={Verbosity bias in preference labeling by large language models},
  author={Saito, Keita and Wachi, Akifumi and Wataoka, Koki and Akimoto, Youhei},
  journal={arXiv preprint arXiv:2310.10076},
  year={2023}
}

@article{dubois2024length,
  title={Length-controlled alpacaeval: A simple way to debias automatic evaluators},
  author={Dubois, Yann and Galambosi, Bal{\'a}zs and Liang, Percy and Hashimoto, Tatsunori B},
  journal={arXiv preprint arXiv:2404.04475},
  year={2024}
}

@article{panickssery2024llm,
  title={Llm evaluators recognize and favor their own generations},
  author={Panickssery, Arjun and Bowman, Samuel R and Feng, Shi},
  journal={arXiv preprint arXiv:2404.13076},
  year={2024}
}

@article{shi2024judging,
  title={Judging the Judges: A Systematic Investigation of Position Bias in Pairwise Comparative Assessments by LLMs},
  author={Shi, Lin and Ma, Weicheng and Vosoughi, Soroush},
  journal={arXiv preprint arXiv:2406.07791},
  year={2024}
}

@article{thakur2024judging,
  title={Judging the Judges: Evaluating Alignment and Vulnerabilities in LLMs-as-Judges},
  author={Thakur, Aman Singh and Choudhary, Kartik and Ramayapally, Venkat Srinik and Vaidyanathan, Sankaran and Hupkes, Dieuwke},
  journal={arXiv preprint arXiv:2406.12624},
  year={2024}
}

@article{chiang2023can,
  title={Can large language models be an alternative to human evaluations?},
  author={Chiang, Cheng-Han and Lee, Hung-yi},
  journal={arXiv preprint arXiv:2305.01937},
  year={2023}
}

@article{liu2023g,
  title={G-eval: Nlg evaluation using gpt-4 with better human alignment},
  author={Liu, Yang and Iter, Dan and Xu, Yichong and Wang, Shuohang and Xu, Ruochen and Zhu, Chenguang},
  journal={arXiv preprint arXiv:2303.16634},
  year={2023}
}

@article{wang2023chatgpt,
  title={Is chatgpt a good nlg evaluator? a preliminary study},
  author={Wang, Jiaan and Liang, Yunlong and Meng, Fandong and Sun, Zengkui and Shi, Haoxiang and Li, Zhixu and Xu, Jinan and Qu, Jianfeng and Zhou, Jie},
  journal={arXiv preprint arXiv:2303.04048},
  year={2023}
}

@article{zhu2310judgelm,
  title={JudgeLM: Fine-tuned Large Language Models are Scalable Judges, October 2023},
  author={Zhu, Lianghui and Wang, Xinggang and Wang, Xinlong},
  journal={URL http://arxiv. org/abs/2310.17631}
}

@article{wang2023pandalm,
  title={Pandalm: An automatic evaluation benchmark for llm instruction tuning optimization},
  author={Wang, Yidong and Yu, Zhuohao and Zeng, Zhengran and Yang, Linyi and Wang, Cunxiang and Chen, Hao and Jiang, Chaoya and Xie, Rui and Wang, Jindong and Xie, Xing and others},
  journal={arXiv preprint arXiv:2306.05087},
  year={2023}
}

@article{li2023generative,
  title={Generative judge for evaluating alignment},
  author={Li, Junlong and Sun, Shichao and Yuan, Weizhe and Fan, Run-Ze and Zhao, Hai and Liu, Pengfei},
  journal={arXiv preprint arXiv:2310.05470},
  year={2023}
}

@article{chen2024humans,
  title={Humans or llms as the judge? a study on judgement biases},
  author={Chen, Guiming Hardy and Chen, Shunian and Liu, Ziche and Jiang, Feng and Wang, Benyou},
  journal={arXiv preprint arXiv:2402.10669},
  year={2024}
}

@article{liusie2023zero,
  title={Zero-shot nlg evaluation through pairware comparisons with llms},
  author={Liusie, Adian and Manakul, Potsawee and Gales, Mark JF},
  journal={arXiv preprint arXiv:2307.07889},
  year={2023}
}

@article{lee2023rlaif,
  title={Rlaif: Scaling reinforcement learning from human feedback with ai feedback},
  author={Lee, Harrison and Phatale, Samrat and Mansoor, Hassan and Lu, Kellie and Mesnard, Thomas and Bishop, Colton and Carbune, Victor and Rastogi, Abhinav},
  journal={arXiv preprint arXiv:2309.00267},
  year={2023}
}

## benchmark
@article{zheng2024judging,
  title={Judging llm-as-a-judge with mt-bench and chatbot arena},
  author={Zheng, Lianmin and Chiang, Wei-Lin and Sheng, Ying and Zhuang, Siyuan and Wu, Zhanghao and Zhuang, Yonghao and Lin, Zi and Li, Zhuohan and Li, Dacheng and Xing, Eric and others},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}

@article{li2024crowdsourced,
  title={From Crowdsourced Data to High-Quality Benchmarks: Arena-Hard and BenchBuilder Pipeline},
  author={Li, Tianle and Chiang, Wei-Lin and Frick, Evan and Dunlap, Lisa and Wu, Tianhao and Zhu, Banghua and Gonzalez, Joseph E and Stoica, Ion},
  journal={arXiv preprint arXiv:2406.11939},
  year={2024}
}

@article{chiang2024chatbot,
  title={Chatbot arena: An open platform for evaluating llms by human preference},
  author={Chiang, Wei-Lin and Zheng, Lianmin and Sheng, Ying and Angelopoulos, Anastasios Nikolas and Li, Tianle and Li, Dacheng and Zhang, Hao and Zhu, Banghua and Jordan, Michael and Gonzalez, Joseph E and others},
  journal={arXiv preprint arXiv:2403.04132},
  year={2024}
}

@article{dubois2024alpacafarm,
  title={Alpacafarm: A simulation framework for methods that learn from human feedback},
  author={Dubois, Yann and Li, Chen Xuechen and Taori, Rohan and Zhang, Tianyi and Gulrajani, Ishaan and Ba, Jimmy and Guestrin, Carlos and Liang, Percy S and Hashimoto, Tatsunori B},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}

@article{lambert2024rewardbench,
  title={Rewardbench: Evaluating reward models for language modeling},
  author={Lambert, Nathan and Pyatkin, Valentina and Morrison, Jacob and Miranda, LJ and Lin, Bill Yuchen and Chandu, Khyathi and Dziri, Nouha and Kumar, Sachin and Zick, Tom and Choi, Yejin and others},
  journal={arXiv preprint arXiv:2403.13787},
  year={2024}
}

## Reward models
@misc{wang2024helpsteer2,
      title={HelpSteer2: Open-source dataset for training top-performing reward models}, 
      author={Zhilin Wang and Yi Dong and Olivier Delalleau and Jiaqi Zeng and Gerald Shen and Daniel Egert and Jimmy J. Zhang and Makesh Narsimhan Sreedhar and Oleksii Kuchaiev},
      year={2024},
      eprint={2406.08673},
      archivePrefix={arXiv},
      primaryClass={id='cs.CL' full_name='Computation and Language' is_active=True alt_name='cmp-lg' in_archive='cs' is_general=False description='Covers natural language processing. Roughly includes material in ACM Subject Class I.2.7. Note that work on artificial languages (programming languages, logics, formal systems) that does not explicitly address natural-language issues broadly construed (natural-language processing, computational linguistics, speech, text retrieval, etc.) is not appropriate for this area.'}
}

## bias mitigation
@article{wang2024eliminating,
  title={Eliminating Position Bias of Language Models: A Mechanistic Approach},
  author={Wang, Ziqi and Zhang, Hanlin and Li, Xiner and Huang, Kuan-Hao and Han, Chi and Ji, Shuiwang and Kakade, Sham M and Peng, Hao and Ji, Heng},
  journal={arXiv preprint arXiv:2407.01100},
  year={2024}
}

## Datasets
## TL;DR summarization
@inproceedings{volske2017tl,
  title={Tl; dr: Mining reddit to learn automatic summarization},
  author={V{\"o}lske, Michael and Potthast, Martin and Syed, Shahbaz and Stein, Benno},
  booktitle={Proceedings of the Workshop on New Frontiers in Summarization},
  pages={59--63},
  year={2017}
}

@article{stiennon2020learning,
  title={Learning to summarize with human feedback},
  author={Stiennon, Nisan and Ouyang, Long and Wu, Jeffrey and Ziegler, Daniel and Lowe, Ryan and Voss, Chelsea and Radford, Alec and Amodei, Dario and Christiano, Paul F},
  journal={Advances in Neural Information Processing Systems},
  volume={33},
  pages={3008--3021},
  year={2020}
}

## flipping noise
@inproceedings{celis2021fair,
  title={Fair classification with noisy protected attributes: A framework with provable guarantees},
  author={Celis, L Elisa and Huang, Lingxiao and Keswani, Vijay and Vishnoi, Nisheeth K},
  booktitle={International Conference on Machine Learning},
  pages={1349--1361},
  year={2021},
  organization={PMLR}
}


## human prefer longer answers
@inproceedings{hart2014perceptions,
  title={Perceptions of answer quality in an online technical question and answer forum},
  author={Hart, Kerry and Sarma, Anita},
  booktitle={Proceedings of the 7th International Workshop on Cooperative and Human Aspects of Software Engineering},
  pages={103--106},
  year={2014}
}

@inproceedings{harper2008predictors,
  title={Predictors of answer quality in online Q\&A sites},
  author={Harper, F Maxwell and Raban, Daphne and Rafaeli, Sheizaf and Konstan, Joseph A},
  booktitle={Proceedings of the SIGCHI Conference on human factors in computing systems},
  pages={865--874},
  year={2008}
}


## Templates
@article{chen2023exploring,
  title={Exploring the use of large language models for reference-free text quality evaluation: An empirical study},
  author={Chen, Yi and Wang, Rui and Jiang, Haiyun and Shi, Shuming and Xu, Ruifeng},
  journal={arXiv preprint arXiv:2304.00723},
  year={2023}
}

@article{zeng2023diversified,
  author       = {Dun Zeng and Yong Dai andPengyu Cheng and Tianhao Hu and Wanshun Chen and
                  Nan Du and Zenglin Xu},
  title        = {On Diversified Preferences of Large Language Model Alignment},
  journal      = {CoRR},
  volume       = {abs/2312.07401},
  year         = {2023},
  url          = {https://doi.org/10.48550/arXiv.2312.07401},
  doi          = {10.48550/ARXIV.2312.07401},
  eprinttype    = {arXiv},
  eprint       = {2312.07401}
}

#### prompt templates used in our study

# scheurer: https://arxiv.org/pdf/2303.16755
@article{scheurer2023training,
  title={Training language models with language feedback at scale},
  author={Scheurer, J{\'e}r{\'e}my and Campos, Jon Ander and Korbak, Tomasz and Chan, Jun Shern and Chen, Angelica and Cho, Kyunghyun and Perez, Ethan},
  journal={arXiv preprint arXiv:2303.16755},
  year={2023}
}

# HH-RLHF-Helpfulness
* bai: https://arxiv.org/pdf/2306.04181
@article{bai2024benchmarking,
  title={Benchmarking foundation models with language-model-as-an-examiner},
  author={Bai, Yushi and Ying, Jiahao and Cao, Yixin and Lv, Xin and He, Yuze and Wang, Xiaozhi and Yu, Jifan and Zeng, Kaisheng and Xiao, Yijia and Lyu, Haozhe and others},
  journal={Advances in Neural Information Processing Systems},
  volume={36},
  year={2024}
}

* guo: https://arxiv.org/pdf/2402.04792
@article{guo2024direct,
  title={Direct language model alignment from online ai feedback},
  author={Guo, Shangmin and Zhang, Biao and Liu, Tianlin and Liu, Tianqi and Khalman, Misha and Llinares, Felipe and Rame, Alexandre and Mesnard, Thomas and Zhao, Yao and Piot, Bilal and others},
  journal={arXiv preprint arXiv:2402.04792},
  year={2024}
}

* wu: https://arxiv.org/pdf/2307.03025
@article{wu2023style,
  title={Style over substance: Evaluation biases for large language models},
  author={Wu, Minghao and Aji, Alham Fikri},
  journal={arXiv preprint arXiv:2307.03025},
  year={2023}
}

* zeng: https://arxiv.org/pdf/2312.07401
@misc{zeng2024diversified,
      title={On Diversified Preferences of Large Language Model Alignment}, 
      author={Dun Zeng and Yong Dai and Pengyu Cheng and Longyue Wang and Tianhao Hu and Wanshun Chen and Nan Du and Zenglin Xu},
      year={2024},
      eprint={2312.07401},
      archivePrefix={arXiv},
      primaryClass={cs.AI}
}

* cheng: https://arxiv.org/pdf/2311.08045
@article{cheng2023adversarial,
  title={Adversarial preference optimization},
  author={Cheng, Pengyu and Yang, Yifan and Li, Jian and Dai, Yong and Du, Nan},
  journal={arXiv preprint arXiv:2311.08045},
  year={2023}
}

* mehta: https://arxiv.org/pdf/2312.00267
@article{mehta2023sample,
  title={Sample Efficient Reinforcement Learning from Human Feedback via Active Exploration},
  author={Mehta, Viraj and Das, Vikramjeet and Neopane, Ojash and Dai, Yijia and Bogunovic, Ilija and Schneider, Jeff and Neiswanger, Willie},
  year={2023}
}

* shen: https://arxiv.org/pdf/2403.07708v2
@article{shen2024improving,
  title={Improving Reinforcement Learning from Human Feedback Using Contrastive Rewards},
  author={Shen, Wei and Zhang, Xiaoying and Yao, Yuanshun and Zheng, Rui and Guo, Hongyi and Liu, Yang},
  journal={arXiv preprint arXiv:2403.07708},
  year={2024}
}

* xu: https://arxiv.org/pdf/2305.18201
@article{xu2023critical,
  title={A critical evaluation of evaluations for long-form question answering},
  author={Xu, Fangyuan and Song, Yixiao and Iyyer, Mohit and Choi, Eunsol},
  journal={arXiv preprint arXiv:2305.18201},
  year={2023}
}


@article{gu2024survey,
  title={A Survey on LLM-as-a-Judge},
  author={Gu, Jiawei and Jiang, Xuhui and Shi, Zhichao and Tan, Hexiang and Zhai, Xuehao and Xu, Chengjin and Li, Wei and Shen, Yinghan and Ma, Shengjie and Liu, Honghao and others},
  journal={arXiv preprint arXiv:2411.15594},
  year={2024}
}

@article{li2024generation,
  title={From generation to judgment: Opportunities and challenges of llm-as-a-judge},
  author={Li, Dawei and Jiang, Bohan and Huang, Liangjie and Beigi, Alimohammad and Zhao, Chengshuai and Tan, Zhen and Bhattacharjee, Amrita and Jiang, Yuxuan and Chen, Canyu and Wu, Tianhao and others},
  journal={arXiv preprint arXiv:2411.16594},
  year={2024}
}

@article{li2024llms,
  title={Llms-as-judges: a comprehensive survey on llm-based evaluation methods},
  author={Li, Haitao and Dong, Qian and Chen, Junjie and Su, Huixue and Zhou, Yujia and Ai, Qingyao and Ye, Ziyi and Liu, Yiqun},
  journal={arXiv preprint arXiv:2412.05579},
  year={2024}
}


